Semi-local string comparison: algorithmic techniques and applications

A classical measure of string comparison is given by the longest common subsequence (LCS) problem on a pair of strings. We consider its generalisation, called the semi-local LCS problem, which arises naturally in many string-related problems. The semi-local LCS problem asks for the LCS scores for each of the input strings against every substring of the other input string, and for every prefix of each input string against every suffix of the other input string. Such a comparison pattern provides a much more detailed picture of string similarity than a single LCS score; it also arises naturally in many string-related problems. In fact, the semi-local LCS problem turns out to be fundamental for string comparison, providing a powerful and flexible alternative to classical dynamic programming. It is especially useful when the input to a string comparison problem may not be available all at once: for example, comparison of dynamically changing strings; comparison of compressed strings; parallel string comparison. The same approach can also be applied to permutation strings, providing efficient solutions for local versions of the longest increasing subsequence (LIS) problem, and for the problem of computing a maximum clique in a circle graph. Furthermore, the semi-local LCS problem turns out to have surprising connections in a few seemingly unrelated fields, such as computational geometry and algebra of semigroups. This work is devoted to exploring the structure of the semi-local LCS problem, its efficient solutions, and its applications in string comparison and other related areas, including computational molecular biology.

==> semi-sparse.tex <==
%%=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=%%
\section{Sparse string comparison}

%%---------------------------------------------------------------------------%%
\subsection{Sparse semi-local LCS}

%%---------------------------------------------------------------------------%%
\begin{framess}


\begin{block}{The LCS problem on permutation strings}
Give LCS score for $a$ vs $b$ 

In each of $a$, $b$ all characters distinct: total $m=n$ matches

Equivalent to
\begin{itemize}
\item \alert{longest increasing subsequence (LIS)} in a string
\item \alert{maximum clique} in a \alert{permutation graph}
\item \alert{maximum planar matching} in an embedded bipartite graph
\end{itemize}
\end{block}

\begin{block}{%
  LCS on permutation strings: running time}
\begin{tabularx}{\textwidth}{@{}llX@{}}
$O(n \log n)$ & & \hfill implicit in [Erd\"os, Szekeres: 1935]\\
& \multicolumn{2}{r@{}}{\hfill [Robinson: 1938; Knuth: 1970; Dijkstra: 1980]}\\
$O(n \log\log n)$ & unit-RAM & \hfill [Chang, Wang: 1992]\\
& & \hfill [Bespamyatnikh, Segal: 2000]
\end{tabularx}
\end{block}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{block}{The semi-local LCS problem on permutation strings}
Give semi-local LCS scores of $a$ vs $b$

In each of $a$, $b$ all characters distinct: total $m=n$ matches

Equivalent to
\begin{itemize}
\item \alert{longest increasing subsequence (LIS)} 
  in every substring of a string
\end{itemize}
\end{block}

\begin{block}{%
  Semi-local LCS on permutation strings: running time}
\begin{tabularx}{\textwidth}{@{}llX@{}}
$O(n^2 \log n)$ & & \hfill naive\\
$O(n^2)$ & restricted & \hfill [Albert+: 2003; Chen+: 2005]\\
$O(n^{1.5} \log n)$ & randomised, restricted & \hfill [Albert+: 2007]\\
$O(n^{1.5})$ & & \hfill [T: 2006]\\
$O(n \log^2 n)$ & & \hfill [T: NEW]
\end{tabularx}
\end{block}

\end{framess}
%%---------------------------------------------------------------------------%%
\extra{%
\begin{framess}

The \alert{sparse LCS} problem: $r$ matches 

Suppose $m=n$, $n \leq r \leq n^2$

\begin{block}{%
  Sparse LCS: running time}
\begin{tabularx}{\textwidth}{@{}lX@{}}
$O(n^2)$ & \hfill naive\\
$O(r \log n)$ & \hfill [Hunt, Szymanski: 1977]\\
$O\bigpa{r \log (n^2/r)}$ & \hfill [Apostolico, Guerra: 1987]
\end{tabularx}
\end{block}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

A simple interpretation using transposition networks

\begin{tikzpicture}[ultra thick,x=0.75cm,y=-0.75cm]
%
\draw (0,0) rectangle (4,4);

\foreach \i in {0.25,0.75,...,4}
  \draw[blue] (\i,0) node[above]{\scriptsize $0$};
\fill[blue!25,fill opacity=0.5] (1.5,0.5) -- ++(0,2.5) -- ++(-0.25,0) --
  ++(0.75,0.75) -- ++(0.75,-0.75) -- ++(-0.25,0) -- ++(0,-2.5) --cycle;
%
\foreach \j in {0.25,0.75,...,4}
  \draw[red] (0,\j) node[left]{\scriptsize $1$};
\fill[red!25,fill opacity=0.5] (0.5,1.5) -- ++(2.5,0) -- ++(0,-0.25) --
  ++(0.75,0.75) -- ++(-0.75,0.75) -- ++(0,-0.25) -- ++(-2.5,0) --cycle;
%
\onslide<2->{%
\draw[thick,blue,opacity=0.5] (2.5,0) -- (3.5,1) -- (3.5,3) -- (4,3.5);
\draw[thick,blue,opacity=0.5] (3,0) -- (4,1);
\draw[thick,red,opacity=0.5] (0,2) -- (1.5,2) -- (3.5,4);
\draw[thick,red,opacity=0.5] (0,2.5) -- (0.5,3) -- (1,3) -- (2,4);}
%
\end{tikzpicture}

%\setlength{\parskip}{1ex minus .2ex}

Implicit \alert{mainstream} of 0s across the network,
split into substreams by 1s moving \alert{diagonally} at matches

For every match, $O(\log n)$ binary search to find its substream

Total work $O(r \log n)$

\end{framess}
}
%%---------------------------------------------------------------------------%%

\newcommand{\doframe}[1]{\draw (o) rectangle +(8,#1);}
\newcommand{\dosplit}[1]{\draw[thin] (o) +(0,#1) -- +(8,#1);}

%%---------------------------------------------------------------------------%%
\begin{framess}

\beginpgfgraphicnamed{f-seaweed-perm-1}%
\begin{tikzpicture}[ultra thick, x=0.5cm, y=-0.5cm]

\alignmentdag{c,f,a,e,d,h,g,b}{d,e,h,c,b,a,f,g}

\path (0,0) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,R,R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,d,D}
  \seaweed{(o) +(3.5, 0)}{r,R,R,R,R}
  \seaweed{(o) +(6.5, 0)}{D,r,R}
  \dosplit{1}}
\onslide<2>{%
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,R,R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,d,D}
  \seaweed{(o) +(3.5, 0)}{r,R,R,R,R}
  \seaweed{(o) +(6.5, 0)}{D,r,R}}
\doframe{2}

\path (0,2) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 1.5)}{R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,R,R,d,D}
  \seaweed{(o) +(1.5, 0)}{D,r,R,R,R,R,R,R}
  \seaweed{(o) +(5.5, 0)}{r,R,R}
  \dosplit{1}}
\onslide<2>{%
  \seaweed{(o) +(0, 1.5)}{R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,R,R,d,r,R,R}
  \seaweed{(o) +(1.5, 0)}{D,r,R,R,R,d}
  \seaweed{(o) +(5.5, 0)}{r,R,R}}
\doframe{2}

\path (0,4) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 1.5)}{R,R,d}
  \seaweed{(o) +(0, 0.5)}{d,D}
  \seaweed{(o) +(0.5, 0)}{r,R,R,R,R,R,R,R}
  \seaweed{(o) +(2.5, 0)}{D,r,R,R,R,R,R}
  \dosplit{1}}
\onslide<2>{%
  \seaweed{(o) +(0, 1.5)}{R,R,d}
  \seaweed{(o) +(0, 0.5)}{d,D}
  \seaweed{(o) +(0.5, 0)}{r,R,R,R,R,R,R,R}
  \seaweed{(o) +(2.5, 0)}{D,r,R,R,R,R,R}}
\doframe{2}

\path (0,6) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,R,R,R,R,d,D}
  \seaweed{(o) +(4.5, 0)}{D,r,R,R,R}
  \seaweed{(o) +(7.5, 0)}{r}
  \dosplit{1}}
\onslide<2>{%
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,d}
  \seaweed{(o) +(0, 0.5)}{R,R,R,R,R,R,R,d,r}
  \seaweed{(o) +(4.5, 0)}{D,r,R,R,d}
  \seaweed{(o) +(7.5, 0)}{r}}
\doframe{2}

\end{tikzpicture}
\endpgfgraphicnamed

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\beginpgfgraphicnamed{f-seaweed-perm-2}%
\begin{tikzpicture}[ultra thick, x=0.5cm, y=-0.5cm]

\alignmentdag{c,f,a,e,d,h,g,b}{d,e,h,c,b,a,f,g}

\path (0,0) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 3.5)}{R,d}
  \seaweed{(o) +(0, 2.5)}{R,R,R,R,R,d,r,R,R}
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,R,R,d,D,D}
  \seaweed{(o) +(0, 0.5)}{R,R,R,d,D,D,D}
  \seaweed{(o) +(1.5, 0)}{D,D,D,r,R,R,R,d}
  \seaweed{(o) +(3.5, 0)}{r,R,R,R,R}
  \seaweed{(o) +(5.5, 0)}{D,D,r,R,R}
  \seaweed{(o) +(6.5, 0)}{D,r,R}
  \dosplit{2}}
\onslide<2>{%
  \seaweed{(o) +(0, 3.5)}{R,d}
  \seaweed{(o) +(0, 2.5)}{R,R,R,R,R,d,r,R,R}
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,R,R,d,r,R}
  \seaweed{(o) +(0, 0.5)}{R,R,R,d,D,D,r,R,d}
  \seaweed{(o) +(1.5, 0)}{D,D,D,r,R,d}
  \seaweed{(o) +(3.5, 0)}{r,R,R,R,R}
  \seaweed{(o) +(5.5, 0)}{D,D,r,d,D}
  \seaweed{(o) +(6.5, 0)}{D,r,R}}
\doframe{4}

\path (0,4) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 3.5)}{R,R,R,R,d}
  \seaweed{(o) +(0, 2.5)}{R,R,R,R,R,R,R,d,r}
  \seaweed{(o) +(0, 1.5)}{R,R,d,D,D}
  \seaweed{(o) +(0, 0.5)}{d,D,D,D}
  \seaweed{(o) +(0.5, 0)}{r,R,R,R,R,R,R,R}
  \seaweed{(o) +(2.5, 0)}{D,r,R,R,R,R,R}
  \seaweed{(o) +(4.5, 0)}{D,D,D,r,R,R,d}
  \seaweed{(o) +(7.5, 0)}{D,D,r}
  \dosplit{2}}
\onslide<2>{%
  \seaweed{(o) +(0, 3.5)}{R,R,R,R,d}
  \seaweed{(o) +(0, 2.5)}{R,R,R,R,R,R,R,d,r}
  \seaweed{(o) +(0, 1.5)}{R,R,d,D,D}
  \seaweed{(o) +(0, 0.5)}{d,D,D,D}
  \seaweed{(o) +(0.5, 0)}{r,R,R,R,R,R,R,R}
  \seaweed{(o) +(2.5, 0)}{D,r,R,R,R,R,R}
  \seaweed{(o) +(4.5, 0)}{D,D,D,r,R,R,d}
  \seaweed{(o) +(7.5, 0)}{D,D,r}}
\doframe{4}

\end{tikzpicture}
\endpgfgraphicnamed

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\beginpgfgraphicnamed{f-seaweed-perm-3}%
\begin{tikzpicture}[ultra thick, x=0.5cm, y=-0.5cm]

\alignmentdag{c,f,a,e,d,h,g,b}{d,e,h,c,b,a,f,g}

\path (0,0) coordinate (o);
\onslide<1|handout:0>{%
  \seaweed{(o) +(0, 7.5)}{R,R,R,R,d}
  \seaweed{(o) +(0, 6.5)}{R,R,R,R,R,R,R,d,r}
  \seaweed{(o) +(0, 5.5)}{R,R,d,D,D}
  \seaweed{(o) +(0, 4.5)}{d,D,D,D}
  \seaweed{(o) +(0, 3.5)}{R,d,D,D,D,D}
  \seaweed{(o) +(0, 2.5)}{R,R,R,R,R,d,r,R,R}
  \seaweed{(o) +(0, 1.5)}{R,R,R,R,R,R,d,r,R}
  \seaweed{(o) +(0, 0.5)}{R,R,R,d,D,D,r,R,d,D,D,D,D}
  \seaweed{(o) +(0.5, 0)}{D,D,D,D,r,R,R,R,R,R,R,R}
  \seaweed{(o) +(1.5, 0)}{D,D,D,r,R,d,D,D,D,D}
  \seaweed{(o) +(2.5, 0)}{D,D,D,D,D,r,R,R,R,R,R}
  \seaweed{(o) +(3.5, 0)}{r,R,R,R,R}
  \seaweed{(o) +(4.5, 0)}{D,D,D,D,D,D,D,r,R,R,d}
  \seaweed{(o) +(5.5, 0)}{D,D,r,d,D,D,D,D,D}
  \seaweed{(o) +(6.5, 0)}{D,r,R}  
  \seaweed{(o) +(7.5, 0)}{D,D,D,D,D,D,D,r}
  \dosplit{4}}
\onslide<2>{%
  \seaweed{(0, 7.5)}{R,R,R,R,d}
  \seaweed{(0, 6.5)}{R,R,R,R,R,R,R,d,r}
  \seaweed{(0, 5.5)}{R,R,d,D,D}
  \seaweed{(0, 4.5)}{d,D,D,D}
  \seaweed{(0, 3.5)}{R,d,r,R,R,R,R,R,R}
  \seaweed{(0, 2.5)}{R,R,R,R,R,d,r,R,R}
  \seaweed{(0, 1.5)}{R,R,R,R,R,R,d,r,R}
  \seaweed{(0, 0.5)}{R,R,R,d,D,D,r,R,d,D,r,R,R}
  \seaweed{(0.5, 0)}{D,D,D,D,r,d,D,D,D}
  \seaweed{(1.5, 0)}{D,D,D,r,R,d,D,r,R,d,D,r,R,d}
  \seaweed{(2.5, 0)}{D,D,D,D,D,r,d,D,D}
  \seaweed{(3.5, 0)}{r,R,R,R,R}
  \seaweed{(4.5, 0)}{D,D,D,D,D,D,D,r,d}
  \seaweed{(5.5, 0)}{D,D,r,d,D,D,D,D,D}
  \seaweed{(6.5, 0)}{D,r,R}
  \seaweed{(7.5, 0)}{D,D,D,D,D,D,r}}
\doframe{8}

\end{tikzpicture}
\endpgfgraphicnamed

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{algorithmblock}{Semi-local LCS on permutation strings: the algorithm}

Divide-and-conquer on the alignment graph

Divide graph (say) horizontally; 
two subproblems of effective size $n/2$

Conquer: seaweed matrix $\odot$-multiplication, time $O(n \log n)$

Overall time $O(n \log^2 n)$

\end{algorithmblock}

\end{framess}
%%---------------------------------------------------------------------------%%
\extra{%
\begin{framess}

The \alert{sparse semi-local LCS} problem: $r$ matches

Suppose $m=n$, $n \leq r \leq n^2$

\begin{block}{%
  Sparse semi-local LCS: running time}
\begin{tabularx}{\textwidth}{@{}lX@{}}
$O(nr^{0.5})$ & \hfill [Krusche, T: 2008]
\end{tabularx}
\end{block}
\pause

Algorithm: divide the alignment graph recursively into square blocks

Recursion base: a block with no matches or a block of size $1$ with a match

Compute each block of size $h > 1$ as a diamond transposition network. 
Can be done in time $O(h)$ instead of the naive $O(h^2)$.

Recursion tree: level $\log_4 r$ dominates, $r$ blocks of size $n/r^{0.5}$

Total work $O(r \cdot n/r^{0.5}) = O(nr^{0.5})$

\end{framess}
}
%%---------------------------------------------------------------------------%%
\subsection{Longest piecewise monotone subsequences}

%%---------------------------------------------------------------------------%%
\begin{framess}

A \alert{$k$-increasing sequence}: 
a concatenation of $k$ increasing sequences

A \alert{$k$-modal sequence}: 
a concatenation of $k$ alternating increasing and decreasing sequences

\begin{block}{%
The longest $k$-increasing ($k$-modal) subsequence problem}

Give the longest $k$-increasing ($k$-modal) subsequence of string $b$
\end{block}

\begin{block}{%
  Longest $k$-increasing ($k$-modal) subsequence: running time}
\begin{tabularx}{\textwidth}{@{}llX@{}}
$O(nk \log n)$ & $k$-modal & \hfill [Demange+: 2007]\\
$O(nk \log n)$ &           & \hfill via [Hunt, Szymanski: 1977] \\
$O(n \log^2 n)$ &      & \hfill [T: NEW]
\end{tabularx}
\end{block}

Main idea: LCS for $\idx^k$ (respectively, $(\idx\ol{\idx})^{k/2}$) vs $b$

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{algorithmblock}{Longest $k$-increasing subsequence: algorithm A}

Sparse LCS for $\idx^k$ vs $b$: time $O(nk \log n)$

\end{algorithmblock}
\pause

\begin{algorithmblock}{Longest $k$-increasing subsequence: algorithm B}

Compute seaweed matrix $P_{\idx,b}$: 
time $O(n \log^2 n)$

Extract three-way submatrix $P^\llcorner_{\idx,b}$: time $O(n \log^2 n)$

Compute matrix $P^\llcorner_{\idx^k,b}$
by $\log k$ instances of seaweed matrix $\odot$-square/multiply:
time $\log k \cdot O(n \log n) = O(n \log^2 n)$

Query the LCS score for $\idx^k$ vs $b$: time negligible

Overall time $O(n \log^2 n)$

\end{algorithmblock}

Algorithm B faster than Algorithm A for $k \geq \log n$

\end{framess}
%%---------------------------------------------------------------------------%%
\subsection{Maximum clique in a circle graph}

\setlength{\unit}{0.8cm}

\renewcommand{\dostep}[2]{%
  \foreach \a/\b in {#1}
    \draw[blue,ultra thick] (\a,\a) rectangle (\b,\b);
  \draw (#2,#2) node[circle, draw, fill, inner sep=0pt, minimum size=4pt]{};}

%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{block}{The maximum clique problem in a circle graph}
Given a circle with $n$ chords,
find the maximum-size subset of pairwise intersecting chords
\end{block}

\begin{columns}[onlytextwidth,T]
%
\column{0.5\textwidth}
%
\beginpgfgraphicnamed{f-circle}%
\begin{tikzpicture}[thick]
%
\draw (0,0) node[circle,draw,dotted,outer sep=0pt,minimum size=4\unit](a){};
%
\draw \foreach \f/\k in {0/0, 30/1, 60/2, 90/3, 120/4, 150/5,
  180/6, 210/7, 240/8, 270/9, 300/10, 330/11}{
  (a.\f) node[circle, fill, inner sep=0pt, minimum size=3pt](a\k){}};
%
\draw (a0) -- (a3) (a1) -- (a10) (a2) -- (a6);
\draw[blue,ultra thick] (a4) -- (a8) (a5) -- (a9) (a7) -- (a11);
\draw (a.345) node[right=0.2cm, inner sep=0pt] {\Large\Leftscissors};
%
\end{tikzpicture}
\endpgfgraphicnamed
%
\column{0.5\textwidth}
%
\beginpgfgraphicnamed{f-circle-int}%
\begin{tikzpicture}[thick, x=0.3cm, y=-0.3cm]
%
\draw[dotted] (0,0) -- (11,11);
%
\foreach \a/\b in {0/3, 1/10, 2/6}
  \draw (\a,\a) rectangle (\b,\b);
%
\dostep{4/8, 5/9, 7/11}{7.5}
%
\end{tikzpicture}
\endpgfgraphicnamed
%
\end{columns}
\pause

Standard reduction to an \alert{interval model}:
cut the circle and lay it out on the line; 
chords become intervals (here drawn as square diagonals)

Chords \alert{intersect} iff intervals \alert{overlap},
i.e.\ intersect without containment

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{block}{%
  Maximum clique in a circle graph: running time}
\begin{tabularx}{\textwidth}{@{}lX@{}}
$\mathit{exp}(n)$ & \hfill naive\\
$O(n^3)$ & \hfill [Gavril: 1973]\\
$O(n^2)$ & \hfill [Rotem, Urrutia: 1981; Hsu: 1985]\\
& \hfill [Masuda+: 1990; Apostolico+: 1992]\\
$O(n^{1.5})$ & \hfill [T: 2006]\\
$O(n \log^2 n)$ & \hfill [T: NEW]
\end{tabularx}
\end{block}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{tikzpicture}[baseline, thick, x=0.3cm, y=-0.3cm]
%
\draw[dotted] (0,0) -- (11,11);
%
\foreach \a/\b in {0/3,1/10,2/6,4/8,5/9,7/11}
  \draw (\a,\a) rectangle (\b,\b);
%
\only<beamer>{%
  \onslide<+>{\dostep{0/3}{0.5}}
  \onslide<+>{\dostep{0/3,1/10}{1.5}}
  \onslide<+>{\dostep{0/3,1/10}{2.5}}
  \onslide<+>{\dostep{2/6}{3.5}}
  \onslide<+>{\dostep{2/6,4/8}{4.5}}
  \onslide<+>{\dostep{2/6,4/8,5/9}{5.5}}
  \onslide<+>{\dostep{4/8,5/9}{6.5}}
  \onslide<+>{\dostep{4/8,5/9,7/11}{7.5}}
  \onslide<+>{\dostep{5/9,7/11}{8.5}}
  \onslide<+>{\dostep{1/10,7/11}{9.5}}
  \onslide<+>{\dostep{7/11}{10.5}}}
%
\only<handout>{\dostep{2/6,4/8,5/9}{5.5}}
%
\end{tikzpicture}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{algorithmblock}{Maximum clique in a circle graph: the algorithm}

\alert{Helly property:} if any set of intervals intersect pairwise,
then they all intersect at a common point

Run semi-local LCS on permutations, build range tree: time $O(n \log^2 n)$

Check all $2n+1$ possible common intersection points

For each point, find a maximum subset 
of covering overlapping segments by a prefix-suffix LCS query:
time $O(n \log^2 n)$

Overall time $O(n \log^2 n) + O(n \log^2 n) = O(n \log^2 n)$

\end{algorithmblock}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{block}{Parameterised maximum clique in a circle graph}
The maximum clique problem in a circle graph, sensitive e.g.\ to 
%
\begin{itemize}
%
\item the number $e$ of edges
\item the size $l$ of maximum clique
\item the thickness $d$ of interval model 
(the maximum number of intervals covering a point)
%
\end{itemize}
\end{block}

We have $l \leq d \leq n$, $e \leq n^2$

\begin{block}{%
  Parameterised maximum clique in a circle graph: running time}
\begin{tabularx}{\textwidth}{@{}lX@{}}
$O(n \log n + e)$            & \hfill [Apostolico+: 1992]\\ \hline
$O(n \log n + nl \log(n/l))$ & \hfill [Apostolico+: 1992]\\ \hline
$O(n \log n + n \log^2 d)$   & \hfill NEW
\end{tabularx}
\end{block}

\end{framess}
%%---------------------------------------------------------------------------%%
\begin{framess}

\begin{algorithmblock}{%
  Parameterised maximum clique in a circle graph: the algorithm}

Run semi-local LCS on diagonal blocks of size $d$, build range trees: 
time $O(n/d \cdot d \log^2 d) = O(n \log^2 d)$

Extend each diagonal block to a quadrant: time $O(n \log^2 d)$

Check all $2n+1$ possible common intersection points: time $O(n \log^2 d)$

Overall time $O(n \log^2 d)$

\end{algorithmblock}

\end{framess}
%%=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=%%

